Extra dimension-inspired models: Z', W', dijet resonances, black hole searches

I give a summary of BSM searches performed by the ATLAS and CMS experiments with an focus on heavy gauge bosons, extra dimensions and quantum black holes. The presented results use data collected during 2012 when the LHC operated at an center of mass energy of $\sqrt{s}$ = 8 TeV.

==> commands.tex <==
% Copyright 2009-2011 Dominik Wagenfuehr <dominik.wagenfuehr@deesaster.org>
% Dieses Dokument unterliegt der Creative-Commons-Lizenz
% "Namensnennung-Weitergabe unter gleichen Bedingungen 3.0 Deutschland"
% [http://creativecommons.org/licenses/by-sa/3.0/de/].

% Pakete
\usepackage[utf8]{inputenc}   % UTF8-Kodierung für Umlaute
\usepackage[T1]{fontenc}      % use TeX encoding then Type 1.
\usepackage{lmodern}          % Bessere Schriftart (ersetzt CM-Schriften)
\usepackage{graphicx}         % Einbindung von Grafiken
\usepackage{fancyhdr}         % eigenes Layout einbinden
\usepackage{pdfpages}         % PDF-Seiten einbinden
\usepackage{xifthen}          % Wenn-dann-Abfragen
\usepackage{charter}          % Charter-Schrift
\usepackage{titlesec}         % Anpassung der Überschriften
\usepackage{longtable}        % Tabellen über Seitenumbruch hinweg
\usepackage{setspace}         % Zeilenabstand festlegen
\usepackage{hyperref}         % Hyperlinks und interne PDF-Verweise

% Layout
\hbadness=10000                % unterdrückt unwichtige Fehlermeldungen
\clubpenalty = 10000           % Keine "Schusterjungen"
\widowpenalty = 10000          % Keine "Hurenkinder"
\displaywidowpenalty = 10000

% Linie im Kopf ausblenden und im Fuß eine feine Linie
\renewcommand*{\headrulewidth}{0pt}
\renewcommand*{\footrulewidth}{0.4pt}

% Überschriftenlayout verändern
\titlespacing{\section}{0mm}{2em}{2em}
\titlespacing{\subsection}{0em}{0em}{0em}
%~ \titleformat{\section}{\normalfont\LARGE\scshape}{}{0mm}{\hspace*{\fill}}
%~ \titleformat{\section}{\normalfont\LARGE\scshape}{}{0mm}{}
\titleformat{\section}{\normalfont\LARGE}{}{0mm}{}
\titleformat{\subsection}{\normalfont\Large\bfseries\scshape}{}{0mm}{}[\vskip-1.5em\hrulefill]
%~ \titleformat{\subsection}{\normalfont\Large\bfseries\scshape}{}{0mm}{}[\hrulefill]
\usepackage[textheight=9.0in,footskip=30pt]{geometry}
% Eigene Fusszeile festlegen, Kopfzeile leeren
\pagestyle{fancy}
\fancyhead{}
\setlength{\footskip}{1.3cm}
\cfoot{\VollerName, \AbsenderStrasse, \AbsenderPLZOrt, \EMail}

% Absender
\newcommand{\Absender}[1][\normalsize]{%
    %~ \rightline{
    \textbf{#1\VollerName} \\
    %~ }
    %~ \rightline{
    \AbsenderStrasse \\
    %~ }
    %~ \rightline{
    \AbsenderPLZOrt \\
    %~ }
    %~ \rightline{
    \Telefon \\
    %~ }
    %~ \rightline{
    \EMail \\
    %~ }
}

% Adressat
\newcommand{\Anschrift}{%
    \textbf{\Firma}\\
    \AnredeKopf{} \AdressatVorname{} \AdressatNachname\\
    \AnschriftStrasse\\
    \AnschriftPLZOrt\\
}

% Makro für Ort und Unterschrift
\newcommand*{\UnterschriftOrt}{%
    %~ \Unterschrift\\
    \vspace{1.2cm}
    \VollerName, \OrtDatum\\
}

% Unterschrift als Bilddatei einfügen
\newcommand*{\Unterschrift}[1][0.1cm]{%
    \hspace*{#1}\includegraphics{\UnterschriftenDatei}%
}

% Tabelle für Lebenslauf
\newlength{\AbstandAbschnitt}
\newboolean{UnterabschnittBegonnen}
\newenvironment{Abschnitt}[1][0em]
{%
    \setlength{\AbstandAbschnitt}{#1}%
    \begin{longtable}{p{0.24\linewidth}p{0.7\linewidth}}%
    \setboolean{UnterabschnittBegonnen}{false}%
}
{%
    \end{longtable}%
    \vspace{\AbstandAbschnitt}%
}

\newenvironment{Abschnitt1}[1][0em]
{%
    \setlength{\AbstandAbschnitt}{#1}%
    \begin{longtable}{p{0.21\linewidth}p{0.74\linewidth}}%
    \setboolean{UnterabschnittBegonnen}{false}%
}
{%
    \end{longtable}%
    \vspace{\AbstandAbschnitt}%
}

% Unterabschnitt in Lebenslauftabelle mit sonstigen Themen
% Achtung, keine Umgebung, sondern ein Kommando!
\newlength{\AbstandUnterabschnitt}
\newcommand{\Unterabschnitt}[3][0em]
{%
    \end{longtable}%
    \ifthenelse{\boolean{UnterabschnittBegonnen}}{%
        \setlength{\AbstandUnterabschnitt}{-5em}%
    }{%
        \setlength{\AbstandUnterabschnitt}{-2em}%
    }%
    \addtolength{\AbstandUnterabschnitt}{#1}%
    \vspace{\AbstandUnterabschnitt}%
    \textit{#2} #3%
    \setboolean{UnterabschnittBegonnen}{true}%
    \begin{longtable}{p{0.25\linewidth}p{0.74\linewidth}}%
    \\[1em]
}

% Anrede im Brief
\newcommand*{\Anrede}{Dear \AnredeText{} \AdressatNachname,}

% Die Grußformel am Anschreibenende
\newcommand{\Grussworte}{%
Please feel free to contact me for any additional questions.

\hspace{3cm}

Kind regards,

%~ \Unterschrift\\[1em]
}

% Betreff
\newcommand*{\Betreff}{\textbf{Application \Bewerberstelle}}

% Etwa Abstand vor dem Ort, um die Seite besser aufteilen zu können.
\newlength{\AbstandVorOrt}
\setlength{\AbstandVorOrt}{1em}

% Abstand zwischen den Adressen im Anschreiben.
\newlength{\AbstandZwischenAdressen}
\setlength{\AbstandZwischenAdressen}{0em}

\newcommand{\AnschreibenKopf}
{%
    % Anschreiben ohne Fuss- oder Kopfzeile
    \thispagestyle{empty}

    % Die Anschreibeseite wird bei Bedarf etwas vergrößert, da es hier keine
    % Fußzeile gibt.
    % \enlargethispage{3cm}
    
    \begin{spacing}{1.05}
        % Meine Anschrift
        \Absender

        % ggf. will man etwas Abstand zwischen den Adressen.
        \vspace*{\AbstandZwischenAdressen}

        % Anschrift der Firma
        \Anschrift

        % ggf. braucht man hier etwas Abstand, je nachdem, wie
        % viel Text man im Anschreiben hat.
        \vspace*{\AbstandVorOrt}

        % Ort und Datum
        \rightline{\OrtDatum}
    \end{spacing}

}

\newcommand{\Anschreiben}
{%
    \AnschreibenKopf
    \begin{spacing}{1.15}
        \Betreff
        \begin{flushleft}
            \Anrede

            \AnschreibenText

            \Grussworte

            \AnschreibenAnlage
        \end{flushleft}
    \end{spacing} 
}


\newcommand{\PersonalInfo}
{% 
    \subsection{Personal data}
    \begin{Abschnitt}
    \textbf{Name} & \VollerName\\
    \textbf{Date of birth} & \Geburtstag \\
    \textbf{Place of birth} & \Geburtsort \\
    \textbf{Marital Status} & \MaritalSatus \\
    \end{Abschnitt}
   
}

\newcommand{\MeineSeite}
{%
    \section{Persönliche Angaben}

    \begin{spacing}{1.3}
        \Absender[\large]
        \vskip0.4em

        %~ \rightline{
        geboren am \Geburtstag \\
        %~ }
        %~ \rightline{
        in \Geburtsort \\
        %~ }
        %~ \vskip1em

        %~ \rightline{
        \Details \\
        %~ }

        %~ \rule{10cm}{0.6pt} \\
        %~ {\large \textbf{Ausbildungsgrad}}\\
        %~ \Ausbildungsgrad\\

        %~ \includegraphics[width=5cm]{\BewerberFoto}\\

    \end{spacing}
}

\newcommand{\MeineMotivation}
{%
    \section{Über mich und meine Motivation}
 
    \begin{spacing}{1.3}
        \begin{flushleft}

        \Motivationstext

        \end{flushleft}
    \end{spacing}
    
    \UnterschriftOrt
}

